Automating Turkish Educational Quiz Generation Using Large Language Models

Crafting quizzes from educational content is a pivotal activity that benefits both teachers and students by reinforcing learning and evaluating understanding. In this study, we introduce a novel approach to generate quizzes from Turkish educational texts, marking a pioneering endeavor in educational technology specifically tailored to the Turkish educational context. We present a specialized dataset, named the Turkish-Quiz-Instruct, comprising an extensive collection of Turkish educational texts accompanied by multiple-choice and short-answer quizzes. This research leverages the capabilities of Large Language Models (LLMs), including GPT-4-Turbo, GPT-3.5-Turbo, Llama-2-7b-chat-hf, and Llama-2-13b-chat-hf, to automatically generate quiz questions and answers from the Turkish educational content. Our work delineates the methodology for employing these LLMs in the context of Turkish educational material, thereby opening new avenues for automated Turkish quiz generation. The study not only demonstrates the efficacy of using such models for generating coherent and relevant quiz content but also sets a precedent for future research in the domain of automated educational content creation for languages other than English. The Turkish-Quiz-Instruct dataset is introduced as a valuable resource for researchers and practitioners aiming to explore the boundaries of educational technology and language-specific applications of LLMs in Turkish. By addressing the challenges of quiz generation in a non-English context specifically Turkish, this study contributes significantly to the field of Turkish educational technology, providing insights into the potential of leveraging LLMs for educational purposes across diverse linguistic landscapes.

==> bib.tex <==
@article{butler2018multiple,
  title={Multiple-choice testing in education: Are the best practices for assessment also good for learning?},
  author={Butler, Andrew C},
  journal={Journal of Applied Research in Memory and Cognition},
  volume={7},
  number={3},
  pages={323--331},
  year={2018},
  publisher={Elsevier}
}


@article{towns2014guide,
  title={Guide to developing high-quality, reliable, and valid multiple-choice assessments},
  author={Towns, Marcy H},
  journal={Journal of Chemical Education},
  volume={91},
  number={9},
  pages={1426--1431},
  year={2014},
  publisher={ACS Publications}
}


@article{dengri2021review,
  title={A review of the quiz, as a new dimension in medical education},
  author={Dengri, Chetna and Gill, Akshay and Chopra, Jayesh and Dengri, Chestha and Koritala, Thoyaja and Khedr, Anwar and Korsapati, Aishwarya Reddy and Adhikari, Ramesh and Jain, Shikha and Zec, Simon and others},
  journal={Cureus},
  volume={13},
  number={10},
  year={2021},
  publisher={Cureus}
}


%%Relatedworks

@article{dugan2022feasibility,
  title={A feasibility study of answer-agnostic question generation for education},
  author={Dugan, Liam and Miltsakaki, Eleni and Upadhyay, Shriyash and Ginsberg, Etan and Gonzalez, Hannah and Choi, Dayheon and Yuan, Chuning and Callison-Burch, Chris},
  journal={arXiv preprint arXiv:2203.08685},
  year={2022}
}


@article{tang2017question,
  title={Question answering and question generation as dual tasks},
  author={Tang, Duyu and Duan, Nan and Qin, Tao and Yan, Zhao and Zhou, Ming},
  journal={arXiv preprint arXiv:1706.02027},
  year={2017}
}

@article{welbl2017crowdsourcing,
  title={Crowdsourcing multiple choice science questions},
  author={Welbl, Johannes and Liu, Nelson F and Gardner, Matt},
  journal={arXiv preprint arXiv:1707.06209},
  year={2017}
}

@article{lai2017race,
  title={Race: Large-scale reading comprehension dataset from examinations},
  author={Lai, Guokun and Xie, Qizhe and Liu, Hanxiao and Yang, Yiming and Hovy, Eduard},
  journal={arXiv preprint arXiv:1704.04683},
  year={2017}
}

@article{xu2022fantastic,
  title={Fantastic Questions and Where to Find Them: FairytaleQA--An Authentic Dataset for Narrative Comprehension},
  author={Xu, Ying and Wang, Dakuo and Yu, Mo and Ritchie, Daniel and Yao, Bingsheng and Wu, Tongshuang and Zhang, Zheng and Li, Toby Jia-Jun and Bradford, Nora and Sun, Branda and others},
  journal={arXiv preprint arXiv:2203.13947},
  year={2022}
}

@inproceedings{wu2023towards,
  title={Towards Data-Effective Educational Question Generation with Prompt-Based Learning},
  author={Wu, Yongchao and Nouri, Jalal and Megyesi, Be{\'a}ta and Henriksson, Aron and Duneld, Martin and Li, Xiu},
  booktitle={Science and Information Conference},
  pages={161--174},
  year={2023},
  organization={Springer}
}

@inproceedings{jia2021eqg,
  title={Eqg-race: Examination-type question generation},
  author={Jia, Xin and Zhou, Wenjie and Sun, Xu and Wu, Yunfang},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={35},
  number={14},
  pages={13143--13151},
  year={2021}
}


@article{steuer2022investigating,
  title={Investigating educational and noneducational answer selection for educational question generation},
  author={Steuer, Tim and Filighera, Anna and Tregel, Thomas},
  journal={IEEE Access},
  volume={10},
  pages={63522--63531},
  year={2022},
  publisher={IEEE}
}

@article{zhao2022educational,
  title={Educational question generation of children storybooks via question type distribution learning and event-centric summarization},
  author={Zhao, Zhenjie and Hou, Yufang and Wang, Dakuo and Yu, Mo and Liu, Chengzhong and Ma, Xiaojuan},
  journal={arXiv preprint arXiv:2203.14187},
  year={2022}
}

@inproceedings{chen2018learningq,
  title={LearningQ: a large-scale dataset for educational question generation},
  author={Chen, Guanliang and Yang, Jie and Hauff, Claudia and Houben, Geert-Jan},
  booktitle={Proceedings of the international AAAI conference on web and social media},
  volume={12},
  number={1},
  year={2018}
}

@inproceedings{gong2022khanq,
  title={Khanq: A dataset for generating deep questions in education},
  author={Gong, Huanli and Pan, Liangming and Hu, Hengchang},
  booktitle={Proceedings of the 29th International Conference on Computational Linguistics},
  pages={5925--5938},
  year={2022}
}

@article{hadifar2023eduqg,
  title={Eduqg: A multi-format multiple-choice dataset for the educational domain},
  author={Hadifar, Amir and Bitew, Semere Kiros and Deleu, Johannes and Develder, Chris and Demeester, Thomas},
  journal={IEEE Access},
  volume={11},
  pages={20885--20896},
  year={2023},
  publisher={IEEE}
}


@inproceedings{kunichika2004automated,
  title={Automated question generation methods for intelligent English learning systems and its evaluation},
  author={Kunichika, Hidenobu and Katayama, Tomoki and Hirashima, Tsukasa and Takeuchi, Akira},
  booktitle={Proc. of ICCE},
  volume={670},
  year={2004}
}


@inproceedings{du2017identifying,
  title={Identifying where to focus in reading comprehension for neural question generation},
  author={Du, Xinya and Cardie, Claire},
  booktitle={Proceedings of the 2017 conference on empirical methods in natural language processing},
  pages={2067--2073},
  year={2017}
}

@article{harrison2018neural,
  title={Neural generation of diverse questions using answer focus, contextual and linguistic features},
  author={Harrison, Vrindavan and Walker, Marilyn},
  journal={arXiv preprint arXiv:1809.02637},
  year={2018}
}

@inproceedings{zhou2018neural,
  title={Neural question generation from text: A preliminary study},
  author={Zhou, Qingyu and Yang, Nan and Wei, Furu and Tan, Chuanqi and Bao, Hangbo and Zhou, Ming},
  booktitle={Natural Language Processing and Chinese Computing: 6th CCF International Conference, NLPCC 2017, Dalian, China, November 8--12, 2017, Proceedings 6},
  pages={662--671},
  year={2018},
  organization={Springer}
}


@article{naeiji2022question,
  title={Question generation using sequence-to-sequence model with semantic role labels},
  author={Naeiji, Alireza},
  year={2022}
}


@article{wang2023multiqg,
  title={Multiqg-ti: Towards question generation from multi-modal sources},
  author={Wang, Zichao and Baraniuk, Richard},
  journal={arXiv preprint arXiv:2307.04643},
  year={2023}
}

@article{zhou2019multi,
  title={Multi-task learning with language modeling for question generation},
  author={Zhou, Wenjie and Zhang, Minghua and Wu, Yunfang},
  journal={arXiv preprint arXiv:1908.11813},
  year={2019}
}

@article{chen2019natural,
  title={Natural question generation with reinforcement learning based graph-to-sequence model},
  author={Chen, Yu and Wu, Lingfei and Zaki, Mohammed J},
  journal={arXiv preprint arXiv:1910.08832},
  year={2019}
}

@inproceedings{chan2019recurrent,
  title={A recurrent BERT-based model for question generation},
  author={Chan, Ying-Hong and Fan, Yao-Chung},
  booktitle={Proceedings of the 2nd workshop on machine reading for question answering},
  pages={154--162},
  year={2019}
}

@inproceedings{wang2022towards,
  title={Towards human-like educational question generation with large language models},
  author={Wang, Zichao and Valdez, Jakob and Basu Mallick, Debshila and Baraniuk, Richard G},
  booktitle={International conference on artificial intelligence in education},
  pages={153--166},
  year={2022},
  organization={Springer}
}

@article{yuan2017machine,
  title={Machine comprehension by text-to-text neural question generation},
  author={Yuan, Xingdi and Wang, Tong and Gulcehre, Caglar and Sordoni, Alessandro and Bachman, Philip and Subramanian, Sandeep and Zhang, Saizheng and Trischler, Adam},
  journal={arXiv preprint arXiv:1705.02012},
  year={2017}
}

@inproceedings{sun2018answer,
  title={Answer-focused and position-aware neural question generation},
  author={Sun, Xingwu and Liu, Jing and Lyu, Yajuan and He, Wei and Ma, Yanjun and Wang, Shi},
  booktitle={Proceedings of the 2018 conference on empirical methods in natural language processing},
  pages={3930--3939},
  year={2018}
}

@inproceedings{ma2020improving,
  title={Improving question generation with sentence-level semantic matching and answer position inferring},
  author={Ma, Xiyao and Zhu, Qile and Zhou, Yanlin and Li, Xiaolin},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={34},
  number={05},
  pages={8464--8471},
  year={2020}
}


@book{lord2012applications,
  title={Applications of item response theory to practical testing problems},
  author={Lord, Frederic M},
  year={2012},
  publisher={Routledge}
}

@article{qiu2020automatic,
  title={Automatic distractor generation for multiple choice questions in standard tests},
  author={Qiu, Zhaopeng and Wu, Xian and Fan, Wei},
  journal={arXiv preprint arXiv:2011.13100},
  year={2020}
}

@inproceedings{uto2023difficulty,
  title={Difficulty-controllable neural question generation for reading comprehension using item response theory},
  author={Uto, Masaki and Tomikawa, Yuto and Suzuki, Ayaka},
  booktitle={Proceedings of the 18th Workshop on Innovative Use of NLP for Building Educational Applications (BEA 2023)},
  pages={119--129},
  year={2023}
}
@article{steuer2021not,
  title={I do not understand what i cannot define: Automatic question generation with pedagogically-driven content selection},
  author={Steuer, Tim and Filighera, Anna and Meuser, Tobias and Rensing, Christoph},
  journal={arXiv preprint arXiv:2110.04123},
  year={2021}
}

@inproceedings{hadifar2023diverse,
  title={Diverse content selection for educational question generation},
  author={Hadifar, Amir and Bitew, Semere Kiros and Deleu, Johannes and Hoste, Veronique and Develder, Chris and Demeester, Thomas},
  booktitle={Proceedings of the 17th Conference of the European Chapter of the Association for Computational Linguistics: Student Research Workshop},
  pages={123--133},
  year={2023}
}


@article{wang2023multi,
  title={Multi-Source Soft Labeling and Hard Negative Sampling for Retrieval Distractor Ranking},
  author={Wang, Jiayun and Rong, Wenge and Bai, Jun and Sun, Zhiwei and Ouyang, Yuanxin and Xiong, Zhang},
  journal={IEEE Transactions on Learning Technologies},
  year={2023},
  publisher={IEEE}
}


@article{srivastava2021question,
  title={Question generation for adaptive education},
  author={Srivastava, Megha and Goodman, Noah},
  journal={arXiv preprint arXiv:2106.04262},
  year={2021}
}
